Towards Debiasing Sentence Representations

As natural language processing methods are increasingly deployed in real-world scenarios such as healthcare, legal systems, and social science, it becomes necessary to recognize the role they potentially play in shaping social biases and stereotypes. Previous work has revealed the presence of social biases in widely used word embeddings involving gender, race, religion, and other social constructs. While some methods were proposed to debias these word-level embeddings, there is a need to perform debiasing at the sentence-level given the recent shift towards new contextualized sentence representations such as ELMo and BERT. In this paper, we investigate the presence of social biases in sentence-level representations and propose a new method, Sent-Debias, to reduce these biases. We show that Sent-Debias is effective in removing biases, and at the same time, preserves performance on sentence-level downstream tasks such as sentiment analysis, linguistic acceptability, and natural language understanding. We hope that our work will inspire future research on characterizing and removing social biases from widely adopted sentence representations for fairer NLP.

==> ACL2020_Debiasing Sentences/figures/alg.tex <==
\newlength{\commentindent}
\setlength{\commentindent}{.3\textwidth}
\makeatletter
\renewcommand{\algorithmiccomment}[1]{\unskip\hfill\makebox[\commentindent][l]{//~#1}\par}
\LetLtxMacro{\oldalgorithmic}{\algorithmic}
\renewcommand{\algorithmic}[1][0]{%
  \oldalgorithmic[#1]%
  \renewcommand{\ALC@com}[1]{%
    \ifnum\pdfstrcmp{##1}{default}=0\else\algorithmiccomment{##1}\fi}%
}
\makeatother

\begin{figure*}
    \begin{minipage}{\linewidth}
    \begin{algorithm}[H]
    \caption{\textsc{Sent-Debias}: a debiasing algorithm for sentence representations.}
    \begin{algorithmic}[1]
        \SUB{\textsc{Sent-Debias}:}
            \STATE Initialize (usually pretrained) sentence encoder $M_\theta$.
            \STATE Define bias attributes (e.g. binary gender $g_{m}$ and $g_f$).
            \STATE Obtain words $\mathcal{D} = \{ (w_1^{(i)}, ..., w_d^{(i)}) \}_{i=1}^m$ indicative of bias attributes (e.g. Table~\ref{words}).
            \STATE $\mathcal{S} = \bigcup_{i=1}^m \textsc{Contextualize}(w_1^{(i)}, ..., w_d^{(i)}) = \{ (s_1^{(i)}, ..., s_d^{(i)}) \}_{i=1}^n$ \COMMENT{words into sentences}
            \FOR{$j \in [d]$}
                \STATE $\mathcal{R}_j = \{ M_\theta( s_j^{(i)} ) \}_{i=1}^n$ \COMMENT{get sentence representations}
            \ENDFOR
            \STATE $\mathbf{V} = \mathbf{PCA}_k \left( \bigcup_{j=1}^d \bigcup_{\mathbf{w} \in \mathcal{R}_j} \left( \mathbf{w} - \bm{\mu}_i \right) \right)$ \COMMENT{compute bias subspace}
            \FOR{each new sentence representation $\mathbf{h}$}
                \STATE $\mathbf{h}_{\mathbf{V}} = \sum_{j=1}^k \langle \mathbf{h}, \mathbf{v}_j \rangle \mathbf{v}_j$ \COMMENT{project onto bias subspace}
                \STATE $\mathbf{\hat{h}} = \mathbf{h} - \mathbf{h}_{\mathbf{V}}$ \COMMENT{subtract projection}
            \ENDFOR
    \end{algorithmic}
    \end{algorithm}
    \end{minipage}
\end{figure*}

==> ACL2020_Debiasing Sentences/figures/fig1.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.0cm]{figures/sst-2-size.png}
    \includegraphics[width=6.0cm]{figures/qnli-size.png}
    \caption{Influence of the number of templates on the effectiveness of bias removal on BERT fine-tuned on SST-2 (left) and BERT fine-tuned on QNLI (right). All templates are from WikiText-2. The solid line represents the mean over different combinations of domains and the shaded area represents the standard deviation. As increasing subsets of data are used, we observe a \textit{decreasing trend} and \textit{lower variance} in average absolute effect size.\vspace{-2mm}}
    \label{fig:sent_size}
\end{figure*}

==> ACL2020_Debiasing Sentences/figures/fig2.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.0cm]{figures/sst-2-domain-fixsize.png}
    \includegraphics[width=6.0cm]{figures/qnli-domain-fixsize.png}
    \caption{Influence of the number of template domains on the effectiveness of bias removal on BERT fine-tuned on SST-2 (left) and BERT fine-tuned on QNLI (right). The domains span the Reddit, SST, POM, WikiText-2 datasets. The solid line is the mean over different combinations of domains and the shaded area is the standard deviation. As more domains are used, we observe a \textit{decreasing trend} and \textit{lower variance} in average absolute effect size.\vspace{-2mm}}
    \label{fig:sent_domain}
\end{figure*}

==> ACL2020_Debiasing Sentences/figures/tsne.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/tsne_plots.pdf}
    \caption{t-SNE plots of average sentence representations of a word across its sentence templates before (left) and after (right) debiasing. After debiasing, non gender-specific concepts (in black) are more equidistant to genders.\vspace{-2mm}}
    \label{fig:tsne}
\end{figure*}

==> ACL2020_Debiasing Sentences/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\usepackage{hyperref}

\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{subcaption}

\usepackage{enumitem}
\setlist{nolistsep}
\setlist[itemize]{noitemsep, topsep=0pt}

\usepackage{times}

\usepackage{graphicx} %
\usepackage{color}

\usepackage{array}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{fancyhdr}
\usepackage{comment}

\setlength{\marginparwidth}{1.5cm}


\newcommand{\thetitle}{Communication-Efficient Learning of Deep Networks \\
from Decentralized Data}
\newcommand{\titlenobreak}{Communication-Efficient Learning of Deep Networks
from Decentralized Data}


\newcommand{\mycaptionof}[2]{\captionof{#1}{#2}}


\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}

\newcommand{\noaistats}[1]{}  %

\definecolor{darkgreen}{rgb}{0,0.4,0.0}
\definecolor{darkblue}{rgb}{0,0.1,0.3}
\definecolor{darkred}{rgb}{0.7,0.0,0.0}


\newcommand{\lbs}{\ensuremath{B}}      %
\newcommand{\all}{\infty}
\newcommand{\lepochs}{\ensuremath{E}}  %
\newcommand{\clientfrac}{\ensuremath{C}}    %
\newcommand{\tnn}{2NN\xspace} %
\newcommand{\xx}{\hspace{-0.01in}\ensuremath{\times}}
\newcommand{\loss}{\ell}
\newcommand{\SUB}[1]{\ENSURE \hspace{-0.15in} \textbf{#1}}
\newcommand{\algfont}[1]{\texttt{#1}}

\renewcommand{\algorithmicensure}{}

\newcommand{\fedavglong}{\algfont{FederatedAveraging}\xspace}
\newcommand{\fedavg}{\algfont{FedAvg}\xspace}
\newcommand{\fedavgshort}{\algfont{FedAvg}\xspace}

\newcommand{\fedsgdlong}{\algfont{FederatedSGD}\xspace}
\newcommand{\fedsgd}{\algfont{FedSGD}\xspace}
\newcommand{\fedsgdshort}{\algfont{FedSGD}\xspace}

\newcommand{\eqdef}{\overset{\text{def}}{=}}
\newcommand{\T}{\rule{0pt}{2.2ex}}
\newcommand{\targetTNN}{97\%\xspace}
\newcommand{\targetCNN}{99\%\xspace}
\newcommand{\targetLSTM}{54\%\xspace}
\newcommand{\nc}{K}
\newcommand{\pp}{\mathcal{P}}


\newlength{\pw}


\newcommand{\BO}{\mathcal{O}}
\newcommand{\qqand}{\qquad \text{and} \qquad}
\newcommand{\qqwhere}{\qquad \text{where} \qquad}
\newcommand{\qqwith}{\qquad \text{with} \qquad}
\newcommand{\grad}{\triangledown}
\newcommand{\h}{\frac{1}{2}}


==> ACL2020_Debiasing Sentences/tables/config.tex <==
%\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}

% \setlength{\tabcolsep}{2pt}
\begin{table}[t]
\fontsize{8.5}{11}\selectfont
\centering
%\fontsize{8.5}{10}\selectfont
%\begin{tabular}{l||*{5}{K{2.4cm}}}
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | l}
\Xhline{3\arrayrulewidth}
Hyper-parameter & Value \\
\Xhline{0.5\arrayrulewidth}
{$\!\begin{aligned}
&\textrm{attention\_probs\_dropout\_prob} \\
&\textrm{hidden\_act} \\
&\textrm{hidden\_dropout\_prob} \\
&\textrm{hidden\_size} \\
&\textrm{initializer\_range} \\ 
&\textrm{intermediate\_size} \\
&\textrm{max\_position\_embeddings} \\
&\textrm{num\_attention\_heads} \\
&\textrm{num\_hidden\_layers} \\
&\textrm{type\_vocab\_size} \\
&\textrm{vocab\_size}
\end{aligned}$} &
{$\!\begin{aligned}
& 0.1 \\
& \textrm{gelu} \\
& 0.1 \\
& 768 \\
& 0.02 \\
& 3072 \\
& 512 \\
& 12 \\
& 12 \\
& 2 \\
& 30522 \end{aligned}$} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Configuration of BERT models, including BERT, BERT$\rightarrow$ SST, and BERT$\rightarrow$ CoLA.}
\label{config}
\end{table}

==> ACL2020_Debiasing Sentences/tables/datasets.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\setlength\tabcolsep{1.5pt}
\begin{tabular}{l | c  c  c  c  c}
\Xhline{3\arrayrulewidth}
Dataset     & Type & Topics & Formality & Length & Samples \\
\Xhline{0.5\arrayrulewidth}
WikiText-2  & written & everything & formal & 24.0 & \makecell{``the mailing contained information about their history\\ and advised people to read several books,\\ which primarily focused on \{\textit{jewish}/\textit{christian}/\textit{muslim}\} history''} \\
\Xhline{0.5\arrayrulewidth}
SST	& written & movie reviews & informal & 19.2 & \makecell{``\{\textit{his}/\textit{her}\} fans walked out muttering words like horrible and terrible, \\but had so much fun dissing the film that they didn't mind the ticket cost.''} \\
\Xhline{0.5\arrayrulewidth}
Reddit & written & \makecell{politics,\\electronics,\\relationships} & informal & 13.6 & \makecell{``roommate cut my hair without my consent,\\ended up cutting \{\textit{himself}/\textit{herself}\} and is threatening to\\ call the police on me''} \\
\Xhline{0.5\arrayrulewidth}
MELD & spoken & comedy TV-series & informal & 8.1 & ``that's the kind of strength that I want in the \{\textit{man}/\textit{woman}\} I love!'' \\
\Xhline{0.5\arrayrulewidth}
POM	& spoken & opinion videos & informal & 16.0 & \makecell{``and \{\textit{his}/\textit{her}\} family is, like, incredibly confused''} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Comparison of the various datasets used to find natural sentence templates. Length represents the average length measured by the number of words in a sentence. Words in italics indicate the words used to estimating the binary gender or multiclass religion subspaces, e.g. (\textit{man}, \textit{woman}), (\textit{jewish}, \textit{christian}, \textit{muslim}). This demonstrates the variety in our naturally occurring sentence templates in terms of topics, formality, and spoken/written text.\vspace{-2mm}}
\label{datasets}
\end{table*}

==> ACL2020_Debiasing Sentences/tables/debias_fix.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]%
\fontsize{8}{11}\selectfont%
\centering
\setlength\tabcolsep{2.2pt}%
\begin{tabular}{l | *{1}{K{2.25cm}} | *{1}{K{2.25cm}} | *{1}{K{2.25cm}} | *{1}{K{2.25cm}} | *{1}{K{2.25cm}}}%
\Xhline{3\arrayrulewidth}%
Test & BERT & BERT post SST-2 & BERT post CoLA & BERT post QNLI & ELMo \\
\Xhline{0.5\arrayrulewidth}
{$\!\begin{aligned}
&\textrm{C6: M/F Names, Career/Family} \\
&\textrm{C6b: M/F Terms, Career/Family} \\
&\textrm{C7: M/F Terms, Math/Arts} \\
&\textrm{C7b: M/F Names, Math/Arts} \\
&\textrm{C8: M/F Terms, Science/Arts} \\ 
&\textrm{C8b: M/F Names, Science/Arts} \\
&\textrm{Multiclass Caliskan} \end{aligned}$} &
{$\!\begin{aligned}
+0.477 &\rightarrow \mathbf{-0.096} \\
\mathbf{+0.108} &\rightarrow -0.437 \\
+0.253 &\rightarrow \mathbf{+0.194} \\
+0.254 &\rightarrow \mathbf{+0.194} \\
+0.399 &\rightarrow \mathbf{-0.075} \\
+0.636 &\rightarrow \mathbf{+0.540} \\
+0.035 &\rightarrow \mathbf{+0.379} \end{aligned}$} &
{$\!\begin{aligned}
\mathbf{+0.036} &\rightarrow -0.109 \\
\mathbf{+0.010} &\rightarrow -0.057 \\
-0.219 &\rightarrow \mathbf{-0.221} \\
+1.153 &\rightarrow \mathbf{-0.755} \\
+0.103 &\rightarrow \mathbf{+0.081} \\
-0.222 &\rightarrow \mathbf{-0.047} \\
+1.200 &\rightarrow \mathbf{+1.000} \end{aligned}$} &
{$\!\begin{aligned}
\mathbf{-0.009} &\rightarrow +0.149 \\
+0.199 &\rightarrow \mathbf{+0.186} \\
\mathbf{+0.268} &\rightarrow +0.311 \\
\mathbf{+0.150} &\rightarrow +0.308 \\
+0.425 &\rightarrow \mathbf{-0.163} \\
\mathbf{+0.032} &\rightarrow -0.192 \\ 
+0.243 &\rightarrow \mathbf{+0.757} \end{aligned}$} &
{$\!\begin{aligned}
-0.261 &\rightarrow \mathbf{-0.054} \\
-0.155 &\rightarrow \mathbf{-0.004} \\
-0.584 &\rightarrow \mathbf{-0.083} \\
\mathbf{-0.581} &\rightarrow -0.629 \\
\mathbf{-0.087} &\rightarrow +0.716 \\
-0.521 &\rightarrow \mathbf{-0.443} \\
& \ \ -  \end{aligned}$} &
{$\!\begin{aligned}
-0.380 &\rightarrow \mathbf{-0.298} \\
-0.345 &\rightarrow \mathbf{-0.327} \\
\mathbf{-0.479} &\rightarrow -0.487 \\
+0.016 &\rightarrow \mathbf{-0.013} \\
\mathbf{-0.296} &\rightarrow -0.327 \\
+0.554 &\rightarrow \mathbf{+0.548} \\
& \ \ - \end{aligned}$} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Debiasing results on BERT and ELMo sentence representations. First six rows measure binary SEAT effect sizes for sentence-level tests, adapted from Caliskan tests. SEAT scores closer to $0$ represent lower bias. C$N$: test from~\citet{caliskan2017semantics} row $N$. The last row measures bias in a multiclass religion setting using MAC~\cite{DBLP:journals/corr/abs-1904-04047} before and after debiasing. MAC score ranges from $0$ to $2$ and closer to $1$ represents lower bias. Results are reported as $x_1 \rightarrow x_2$ where $x_1$ represents score before debiasing and $x_2$ after, with lower bias score in bold. Our method reduces bias of BERT and ELMo for the majority of binary and multiclass tests.}
%\vspace{-6mm}}
\label{debias}
\end{table*}

==> ACL2020_Debiasing Sentences/tables/debias_fix_old.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]%
\fontsize{8}{11}\selectfont%
\centering
\setlength\tabcolsep{2.2pt}%
\begin{tabular}{l | *{1}{K{2.35cm}} | *{1}{K{2.35cm}} | *{1}{K{2.35cm}} | *{1}{K{2.35cm}} | *{1}{K{2.35cm}}}%
\Xhline{3\arrayrulewidth}%
Test & BERT & BERT post SST-2 & BERT post CoLA & BERT post QNLI & ELMo \\
\Xhline{0.5\arrayrulewidth}
{$\!\begin{aligned}
&\textrm{C6: M/F Names, Career/Family} \\
&\textrm{C6b: M/F Terms, Career/Family} \\
&\textrm{C7: M/F Terms, Math/Arts} \\
&\textrm{C7b: M/F Names, Math/Arts} \\
&\textrm{C8: M/F Terms, Science/Arts} \\ 
&\textrm{C8b: M/F Names, Science/Arts} \\
&\textrm{Multiclass Caliskan} \end{aligned}$} &
{$\!\begin{aligned}
+0.158 &\rightarrow \mathbf{-0.095} \\
\mathbf{+0.168} &\rightarrow +0.121 \\
+0.542 &\rightarrow \mathbf{+0.082} \\
+0.434 &\rightarrow \mathbf{-0.289} \\
+0.297 &\rightarrow \mathbf{-0.362} \\
+0.063 &\rightarrow \mathbf{-0.047} \\
+0.035 &\rightarrow \mathbf{+0.379} \end{aligned}$} &
{$\!\begin{aligned}
+0.126 &\rightarrow \mathbf{+0.026} \\
+0.232 &\rightarrow \mathbf{-0.160} \\
\mathbf{-0.033} &\rightarrow -0.280 \\
-1.142 &\rightarrow \mathbf{+0.161} \\
-0.148 &\rightarrow \mathbf{+0.020} \\
-0.089 &\rightarrow \mathbf{+0.045} \\
+1.200 &\rightarrow \mathbf{+1.000} \end{aligned}$} &
{$\!\begin{aligned}
-0.293 &\rightarrow \mathbf{-0.036} \\
\mathbf{+0.052} &\rightarrow +0.065 \\
+0.288 &\rightarrow \mathbf{+0.074} \\
-0.176 &\rightarrow \mathbf{+0.076} \\
\mathbf{+0.258} &\rightarrow +0.521 \\
-0.470 &\rightarrow \mathbf{-0.290} \\
+0.243 &\rightarrow \mathbf{+0.757} \end{aligned}$} &
{$\!\begin{aligned}
\mathbf{-0.027} &\rightarrow +0.226 \\
+0.111 &\rightarrow \mathbf{-0.052} \\
+0.377 &\rightarrow \mathbf{+0.010} \\
-0.404 &\rightarrow \mathbf{-0.082} \\
+0.332 &\rightarrow \mathbf{-0.305} \\
-0.272 &\rightarrow \mathbf{+0.001} \\
& \ \ -  \end{aligned}$} &
{$\!\begin{aligned}
-0.380 &\rightarrow \mathbf{-0.298} \\
-0.345 &\rightarrow \mathbf{-0.327} \\
\mathbf{-0.479} &\rightarrow -0.487 \\
+0.016 &\rightarrow \mathbf{-0.013} \\
\mathbf{-0.296} &\rightarrow -0.327 \\
+0.554 &\rightarrow \mathbf{+0.548} \\
& \ \ - \end{aligned}$} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Debiasing results on BERT and ELMo sentence representations. First six rows measure binary SEAT effect sizes for sentence-level tests, adapted from Caliskan tests. SEAT scores closer to $0$ represent lower bias. C$N$: test from~\citet{caliskan2017semantics} row $N$. The last row measures bias in a multiclass religion setting using MAC~\cite{DBLP:journals/corr/abs-1904-04047} before and after debiasing. MAC score ranges from $0$ to $2$ and closer to $1$ represents lower bias. Results are reported as $x_1 \rightarrow x_2$ where $x_1$ represents score before debiasing and $x_2$ after. Better effect sizes are highlighted in bold. Our method reduces bias of BERT and ELMo for the majority of binary and multiclass tests.}
\label{debias}
\end{table*}

==> ACL2020_Debiasing Sentences/tables/downstream.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\centering
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l | c  c | c  c}
\Xhline{3\arrayrulewidth}
\multicolumn{1}{l|}{Test} & BERT & Less biased BERT & ELMo & Less biased ELMo \\
\Xhline{0.5\arrayrulewidth}
SST-2& $92.7$ & $89.1$ & $89.6$ & $90.0$ \\
CoLA & $57.6$ & $55.4$ & $39.1$ & $37.1$ \\
QNLI & $91.3$ & $90.6$ & - & - \\
\Xhline{3\arrayrulewidth}%
\end{tabular}
\caption{We test the effect of \textsc{Sent-Debias} on both single sentence (BERT and ELMo on SST-2, CoLA) and paired sentence (BERT on QNLI) downstream tasks. The performance (higher is better) of debiased BERT and ELMo sentence representations on downstream tasks is not hurt by the debiasing step.\vspace{-4mm}}
\label{downstream}
\end{table}

==> ACL2020_Debiasing Sentences/tables/word_baseline.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\centering
%\fontsize{8.5}{10}\selectfont
%\begin{tabular}{l||*{5}{K{2.4cm}}}
\setlength\tabcolsep{2.5pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Debiasing Method & Ave. Abs. Effect Size\\
\Xhline{0.5\arrayrulewidth}
BERT original~\citep{DBLP:journals/corr/abs-1810-04805} & $+0.354$\\
FastText~\citep{bojanowski2016enriching} & $+0.565$\\
BERT word~\citep{bolukbasi2016man} & $+0.861$\\
BERT simple~\citep{DBLP:journals/corr/abs-1903-10561} & $+0.298$\\
\textsc{Sent-Debias} BERT (ours) & $\mathbf{+0.256}$\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Comparison of various debiasing methods on sentence embeddings. FastText~\citep{bojanowski2016enriching} (and BERT word) derives debiased sentence embeddings with an average of debiased FastText (and BERT) word embeddings using word-level debiasing methods~\citep{bolukbasi2016man}. BERT simple adapts~\citet{DBLP:journals/corr/abs-1903-10561} by using simple templates to debias BERT representations. \textsc{Sent-Debias} BERT represents our method using diverse templates. We report the average absolute effect size across all Caliskan tests. Average scores closer to $0$ represent lower bias.\vspace{-4mm}}
\label{simple}
\end{table}

==> ACL2020_Debiasing Sentences/tables/words.tex <==
\begin{table}[!tbp]
    \fontsize{9}{11}\selectfont
    \begin{minipage}{.4\linewidth}
        \centering
        \setlength\tabcolsep{3.5pt}
        \begin{tabular}{c}
        \Xhline{3\arrayrulewidth}
        Binary Gender\\
        \Xhline{0.5\arrayrulewidth}
        man, woman \\
        he, she \\
        father, mother \\
        son, daughter \\
        \Xhline{3\arrayrulewidth}
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.6\linewidth}
        \centering
        \setlength\tabcolsep{3.5pt}
        \begin{tabular}{c}
        \Xhline{3\arrayrulewidth}
        Multiclass Religion\\
        \Xhline{0.5\arrayrulewidth}
        jewish, christian, muslim \\
        torah, bible, quran \\
        synagogue, church, mosque \\
        rabbi, priest, imam \\
        \Xhline{3\arrayrulewidth}
        \end{tabular}
    \end{minipage}
    \caption{Examples of word pairs to estimate the binary gender bias subspace and the $3$-class religion bias subspace in our experiments.\vspace{-4mm}}
    \label{words}
\end{table}

==> tables/debias_fix_old.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]%
\fontsize{8}{11}\selectfont%
\centering
\setlength\tabcolsep{2.2pt}%
\begin{tabular}{l | *{1}{K{2.35cm}} | *{1}{K{2.35cm}} | *{1}{K{2.35cm}} | *{1}{K{2.35cm}} | *{1}{K{2.35cm}}}%
\Xhline{3\arrayrulewidth}%
Test & BERT & BERT post SST-2 & BERT post CoLA & BERT post QNLI & ELMo \\
\Xhline{0.5\arrayrulewidth}
{$\!\begin{aligned}
&\textrm{C6: M/F Names, Career/Family} \\
&\textrm{C6b: M/F Terms, Career/Family} \\
&\textrm{C7: M/F Terms, Math/Arts} \\
&\textrm{C7b: M/F Names, Math/Arts} \\
&\textrm{C8: M/F Terms, Science/Arts} \\ 
&\textrm{C8b: M/F Names, Science/Arts} \\
&\textrm{Multiclass Caliskan} \end{aligned}$} &
{$\!\begin{aligned}
+0.158 &\rightarrow \mathbf{-0.095} \\
\mathbf{+0.168} &\rightarrow +0.121 \\
+0.542 &\rightarrow \mathbf{+0.082} \\
+0.434 &\rightarrow \mathbf{-0.289} \\
+0.297 &\rightarrow \mathbf{-0.362} \\
+0.063 &\rightarrow \mathbf{-0.047} \\
+0.035 &\rightarrow \mathbf{+0.379} \end{aligned}$} &
{$\!\begin{aligned}
+0.126 &\rightarrow \mathbf{+0.026} \\
+0.232 &\rightarrow \mathbf{-0.160} \\
\mathbf{-0.033} &\rightarrow -0.280 \\
-1.142 &\rightarrow \mathbf{+0.161} \\
-0.148 &\rightarrow \mathbf{+0.020} \\
-0.089 &\rightarrow \mathbf{+0.045} \\
+1.200 &\rightarrow \mathbf{+1.000} \end{aligned}$} &
{$\!\begin{aligned}
-0.293 &\rightarrow \mathbf{-0.036} \\
\mathbf{+0.052} &\rightarrow +0.065 \\
+0.288 &\rightarrow \mathbf{+0.074} \\
-0.176 &\rightarrow \mathbf{+0.076} \\
\mathbf{+0.258} &\rightarrow +0.521 \\
-0.470 &\rightarrow \mathbf{-0.290} \\
+0.243 &\rightarrow \mathbf{+0.757} \end{aligned}$} &
{$\!\begin{aligned}
\mathbf{-0.027} &\rightarrow +0.226 \\
+0.111 &\rightarrow \mathbf{-0.052} \\
+0.377 &\rightarrow \mathbf{+0.010} \\
-0.404 &\rightarrow \mathbf{-0.082} \\
+0.332 &\rightarrow \mathbf{-0.305} \\
-0.272 &\rightarrow \mathbf{+0.001} \\
& \ \ -  \end{aligned}$} &
{$\!\begin{aligned}
-0.380 &\rightarrow \mathbf{-0.298} \\
-0.345 &\rightarrow \mathbf{-0.327} \\
\mathbf{-0.479} &\rightarrow -0.487 \\
+0.016 &\rightarrow \mathbf{-0.013} \\
\mathbf{-0.296} &\rightarrow -0.327 \\
+0.554 &\rightarrow \mathbf{+0.548} \\
& \ \ - \end{aligned}$} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Debiasing results on BERT and ELMo sentence representations. First six rows measure binary SEAT effect sizes for sentence-level tests, adapted from Caliskan tests. SEAT scores closer to $0$ represent lower bias. C$N$: test from~\citet{caliskan2017semantics} row $N$. The last row measures bias in a multiclass religion setting using MAC~\cite{DBLP:journals/corr/abs-1904-04047} before and after debiasing. MAC score ranges from $0$ to $2$ and closer to $1$ represents lower bias. Results are reported as $x_1 \rightarrow x_2$ where $x_1$ represents score before debiasing and $x_2$ after. Better effect sizes are highlighted in bold. Our method reduces bias of BERT and ELMo for the majority of binary and multiclass tests.}
\label{debias}
\end{table*}
